On the Overlooked Significance of Underutilized Contextual Features in Recent News Recommendation Models

Personalized news recommendation aims to provide attractive articles for readers by predicting their likelihood of clicking on a certain article. To accurately predict this probability, plenty of studies have been proposed that actively utilize content features of articles, such as words, categories, or entities. However, we observed that the articles' contextual features, such as CTR (click-through-rate), popularity, or freshness, were either neglected or underutilized recently. To prove that this is the case, we conducted an extensive comparison between recent deep-learning models and naive contextual models that we devised and surprisingly discovered that the latter easily outperforms the former. Furthermore, our analysis showed that the recent tendency to apply overly sophisticated deep-learning operations to contextual features was actually hindering the recommendation performance. From this knowledge, we design a purposefully simple contextual module that can boost the previous news recommendation models by a large margin.

==> sections/boosting_subsections/boosting.tex <==
Following \cite{hyperconnectboosting}, we chose gradient boosting as our method. We constructed tabular data with click/non-click data as label column and contextual features as feature columns. Then we used CatBoost library \cite{catboost} to train and evaluate on those tables. We ensured that metrics from deep-learning evaluation and gradient boosting evaluation could be compared apple-to-apple.

==> sections/deeplearning_subsections/model_figure.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{sections/figures/contextmodule.pdf}
  \caption{(a) Our approach to enhance previous content-based news recommendation models with a modular attachment of a context module. (b) Our suggestion for the context module.}
  \Description[Test Desc]{Test Description}
  \label{fig:context_module}
\end{figure*}

==> sections/experiments.tex <==
\subsection{Datasets \& Evaluation}
\input{sections/experiments_subsection/datasets}

\subsection{Baselines}
\input{sections/experiments_subsection/baselines}

% \subsection{Experiment Setup}
% \input{sections/experiments_subsection/experiment_setup}

\subsection{Implementation Details}
\input{sections/experiments_subsection/implementation_details}

\subsection{Performance Comparison}
\input{sections/experiments_subsection/performance_comparison}

\subsection{Ablation Studies}
\input{sections/experiments_subsection/ablation}

==> sections/experiments_subsection/ablation.tex <==
%  Tower combination 실험 \\
%  Information Bottleneck 증명 혹은 measure하는 실험 (차후 구체화) \\
%  우리의 user-modeling개선이 news-modeling 모듈에 대해 orthogonal 함을 보이기 (news encoder 갈아끼워보기) \\
%  그냥 impression eval set에서도 성능 개선 있음을 보이기? \\
%  alpha 등의 파라미터 변화에 따른 성능 변화 실험 \\
%  model debugging (attention heatmaps or in-depth analysis of what our model is doing) \\
%  embedding (or encoder result) projection plot \\

\subsubsection{Effectiveness of each tower}
\label{combinationablation}


\begin{table}[]
\caption{Contribution of each type of tower on Small dataset. (N=NDCG, R=Recall)}
\Description[Description]{Description}
\label{tab:combination}
\begin{tabular}{l|rrrr}
\toprule
  & \Delta \text{N}@10     & N@10 Improv.      & \Delta \text{R}@10     & R@10 Improv.     \\ \midrule
+\textbf{w} & 0.0118 & 4.85\% & 0.0146 & 3.37\% \\
+\textbf{p} & 0.0115 & 4.79\% & 0.0152 & 3.46\% \\
+\textbf{c} & 0.0080 & 2.82\% & 0.0131 & 2.53\% \\
+\textbf{s} & 0.0037 & 1.66\% & 0.0065 & 1.55\% \\
+\textbf{t} & 0.0291 & 9.78\% & 0.0432 & 7.91\% \\
+\textbf{f} & 0.0050 & 1.73\% & 0.0047 & 0.95\% \\
\bottomrule
\end{tabular}
\end{table}


To assess the contribution of each type of tower, we conducted the following ablation study. First, we evaluated the performance of every combination between $\textbf{(wpcstf)}^\textbf{0}$ and $\textbf{(wpcstf)}^\textbf{2}$ on the \textbf{Small} dataset (in other words, all combinations where the number of each tower is within [0,2] (e.g. \textbf{wcct})). Ignoring $\textbf{(wpcstf)}^\textbf{0}$ since it is an empty model, we have $3^6 - 1 = 728$ such combinations. We used default hyperparameters for each experiment.  Next, for each type of tower (e.g. \textbf{w}), we gathered all pairs of combinations that differ only in the count of that type of tower by 1 (e.g. $\textbf{wpc} \rightarrow \textbf{wwpc}$). Then we measured the performance improvement in each pair in terms of NDCG@10 and Recall@10. Table \ref{tab:combination} shows the average of those results. We can observe that each type of tower is useful because they all improve the performance when added. We can also observe that the contribution of \textbf{t} is the largest, which shows that trend is a valuable signal when it comes to recommending news articles. Subsequently, semantic towers were important. It is interesting to note that while $\mathcal{T}^{word}$ brings larger improvement in NDCG@10 than $\mathcal{T}^{personal}$, the reverse is true in Recall@10. This shows that they bring different gains to the system despite operating on the same semantic features. In the categorical towers, $\mathcal{T}^{cat}$ was more helpful than $\mathcal{T}^{subcat}$, which is understandable since people's interest in bigger categories such as economy tend to be more apparent and persistent than their interest in smaller categories such as a real estates. Finally, $\mathcal{T}^{fresh}$ improved the framework's capacity by the least amount, possibly because the candidate items consisted of similarly fresh articles.

\subsubsection{Effect of tower combination}

In the previous section, we studied the effect of adding a certain type of tower to the framework. Since adding a tower brings more parameters to the system, the performance improvement might be viewed only as the result of having more parameters. To show that this is not the case, we conducted the following study. First, we used \textbf{wpcstf} as the baseline. Then we compared its performance with $\textbf{w}^\textbf{6}$, $\textbf{p}^\textbf{6}$, $\textbf{c}^\textbf{6}$, $\textbf{s}^\textbf{6}$, $\textbf{t}^\textbf{6}$, and $\textbf{f}^\textbf{6}$. Note that by using six towers each, the number of parameters is kept at a similar level with the baseline. These models were evaluated on the \textbf{Small} dataset. The results are shown on the left side of Table \ref{tab:all6}. In addition, since using many number of the same tower can be prone to overfitting as shown in section \ref{section:numblocks}, we also included the best performance among 1 to 6 towers (e.g. $\textbf{w}^\textbf{1}$, ..., $\textbf{w}^\textbf{6}$) to be fair. Their results are shown on the right side of the table.

We can observe that the baseline far outperforms the ones that only use a single type of tower on either side of the table (some perform much worse when employed alone). Given that these models use similar level of parameters, the difference can only be explained by the diversity in the towers. Each type of tower captures a different aspect of users and news articles, which cannot be captured by other types of towers no matter how many of them are stacked. This proves our claim that the performance of the previous news recommendation framework was hindered by its limited use of features and encoders, and that enhancement such as \textbf{NR-MOST} suggested in this paper is indeed necessary. It also shows that our framework is open to more kinds of features and towers which will improve the performance as long as they reveal certain aspects of the users and the articles that haven't been captured before.

\begin{table}[]
\caption{Effect of using a combination of towers on Small dataset (N=NDCG, R=Recall).}
\Description[Description]{Description}
\label{tab:all6}
\begin{tabular}{r|rr|rr}
\toprule
  & N@10     & R@10    & Best N@10    & Best R@10    \\ \midrule
\textbf{w}^\textbf{6} & 0.2865 & 0.5513 & 0.3159 & 0.5721 \\
\textbf{p}^\textbf{6} & 0.2972 & 0.5585 & 0.3133 & 0.5705 \\
\textbf{c}^\textbf{6} & 0.1629 & 0.3438 & 0.1695 & 0.3526 \\
\textbf{s}^\textbf{6} & 0.2141 & 0.4327 & 0.2181 & 0.4367 \\
\textbf{t}^\textbf{6} & 0.2345 & 0.4808 & 0.2399 & 0.4816 \\
\textbf{f}^\textbf{6} & 0.1634 & 0.3245 & 0.1644 & 0.3245 \\ \midrule
\textbf{wpcstf} & \textbf{0.4026} & \textbf{0.7083} & \textbf{0.4026} & \textbf{0.7083}  \\
\bottomrule
\end{tabular}
\end{table}



% \begin{table}[]
% \caption{Effect of using a combination of towers on Small dataset}
% \Description[Description]{Description}
% \label{tab:all6}
% \begin{tabular}{r|rr}
% \toprule
%   & NDCG@10     & Recall@10    \\ \midrule
% \textbf{w}^\textbf{6} & 0.2865 & 0.5513 \\
% \textbf{p}^\textbf{6} & 0.2972 & 0.5585 \\
% \textbf{c}^\textbf{6} & 0.1629 & 0.3438 \\
% \textbf{s}^\textbf{6} & 0.2141 & 0.4327 \\
% \textbf{t}^\textbf{6} & 0.2345 & 0.4808 \\
% \textbf{f}^\textbf{6} & 0.1634 & 0.3245 \\ \midrule
% \textbf{wpcstf} & \textbf{0.4026} & \textbf{0.7083} \\
% \bottomrule
% \end{tabular}
% \end{table}


\subsubsection{Effect of the interaction layer and the score linear layer}

In line with the previous section, we further study the effect of the interactions between multiple towers. Recall that in our framework, as shown in Figure \ref{fig:ourframework}, we have largely two layers that combine the effect of multiple towers. We first have an interaction layer, as shown in Figure \ref{fig:ourframework} (d), which seeks to model the complicated relationships between the representations from each tower by feed forward networks. We then have a score linear layer, as shown in Figure \ref{fig:ourframework} (e), which combines the result from the interaction layer and the scores from each tower by weighted sum to make the final prediction. Table \ref{tab:interaction} shows an ablation study on these two components. We ran three experiments with the combination of $\textbf{(wpcstf)}^{\textbf{2}}$ on the \textbf{Small} dataset. However, the first row was done without the score layer (only with the interaction layer), and the second row was done vice versa. The large performance drop in the first row shows that the final score combination is indeed necessary and the interaction layer alone is not enough. More importantly, the performance drop in the second row shows that interaction layer is also a crucial component in our framework. This proves our claim that simple operations such as dot product used in the previous frameworks are not enough to model the interactions between the representations.


\begin{table}[]
\caption{Effect of removing the score layer and the interaction layer}
\Description[Description]{Description}
\label{tab:interaction}
\begin{tabular}{r|rr}
\toprule
  & NDCG@10     & Recall@10    \\ \midrule
Without score layer & 0.3804 & 0.6819 \\
Without interaction layer & 0.4009 & 0.6987 \\ \midrule
\textbf{(wpcstf)}^{\textbf{2}} & \textbf{0.4089} & \textbf{0.7276} \\
\bottomrule
\end{tabular}
\end{table}



\subsubsection{Effect of having a separate categorical tower}

Recall that \textbf{NR-MOST} is not the only model that makes use of categorical features. Among our baselines, \textbf{NAML}~\cite{NAML} and \textbf{LSTUR}~\cite{an2019} incorporate categorical features into their news encoders. However, the big difference in our framework is that we have separate towers dedicated to categorical features. To show that this method is better than having the same tower process multiple features, we conducted the following ablation study. First, inspired by \textbf{NAML}, we devised a simple tower $\mathcal{T}^{mixed}$ (denoted by \textbf{m}) which differs from $\mathcal{T}^{word}$ only in its news encoder. In the news encoder of $\mathcal{T}^{mixed}$, the semantic vector of an article is produced by $\textrm{Enc}_{\textrm{(Mult, Add)}}$ as in the news encoder of $\mathcal{T}^{word}$. In addition, it obtains vectors for (sub)category of the article by embedding look-ups and dense layers. These three vectors are combined into a single vector by additive attention operation. Notice that the overall structure resembles the news encoder used in \textbf{NAML}.

\begin{table}[H]
\caption{Effect of having a separate dedicated categorical tower}
\Description[Description]{Description}
\label{tab:separate}
\begin{tabular}{r|rr}
\toprule
  & NDCG@10     & Recall@10    \\ \midrule
\textbf{mmmptf} & 0.3917 & 0.7043 \\ \midrule
\textbf{wpcstf} & \textbf{0.4026} & \textbf{0.7083} \\
\bottomrule
\end{tabular}
\end{table}

Next, since $\mathcal{T}^{mixed}$ can be said to be functioning as a mixture of $\mathcal{T}^{word}$, $\mathcal{T}^{cat}$, and $\mathcal{T}^{subcat}$, we made a variant of \textbf{wpcstf} by replacing all occurrences of \textbf{w}, \textbf{c}, and \textbf{s} with \textbf{m} to get \textbf{mmmptf}. The performance of this variant is shown in Table \ref{tab:separate}. We can observe that the performance drops when we replace the specialized towers with towers that have mixed purpose, even when the overall parameter size and the model structure remain similar. Also, note that \textbf{mmmptf} still outperforms all of the baseline models because it also uses all of the features we devised. This proves that (a) it is beneficial to have specialized towers as in \textbf{NR-MOST} because using the same tower for multiple features leads to information bottleneck, and that (b) our proposed framework still brings significant performance improvement even when the mixed towers from the baseline models are employed.

\subsubsection{Importance of temporal features}

Although the overall structure of \textbf{NR-MOST} is what we emphasized the most so far, we also regard the novelty of our temporal features and encoders as important contributions in terms of performance gain. To show the power of temporal features independently from \textbf{NR-MOST}, we tried adding the \texttt{trend} feature to the \textbf{DeepFM} model since it is a general factorization machine that allows any number of features. To obtain the \texttt{trend} feature in the vector form from the scalar value $\texttt{trend}(n,t)$, we used $\log(1+x)$ operation and dense layers .


\begin{table}[H]
\caption{Impact of temporal features on DeepFM}
\Description[Description]{Description}
\label{tab:deepfmtrendsmall}
\begin{tabular}{r|rrr}
\toprule
  & \textbf{DeepFM}     & \textbf{DeepFM+trend}     & Improv.  \\ \midrule
\textbf{Small} NDCG@10 & 0.2463 & \textbf{0.3273} & 32.89\% \\
\textbf{Small} Recall@10 & 0.4768 & \textbf{0.6178} & 29.57\% \\
\textbf{Large} NDCG@10 & 0.2497 & \textbf{0.3331} & 33.40\% \\
\textbf{Large} Recall@10 & 0.5036 & \textbf{0.6361} & 26.31\% \\
\bottomrule
\end{tabular}
\end{table}

Table \ref{tab:deepfmtrendsmall} shows the performance gain in both \textbf{Small} and \textbf{Large} datasets. We can see that the temporal features as we devised them contain valuable information for news recommendation since they boost the performance by a large amount. Also, even though the performance of \textbf{DeepFM+trend} improves significantly, it still underperforms \textbf{NR-MOST} and some of the baselines. This shows that temporal features alone are not enough.


\subsubsection{Effect of $\alpha$}

\begin{figure}[H]
  \centering
  \includegraphics[width=\linewidth]{sections/figures/alpha.pdf}
  \caption{The influence of $\alpha$ on the performance of \textbf{POP} (left) and \textbf{NR-MOST} (right)}
  \Description[Test Desc]{Test Description}
  \label{fig:alpha}
\end{figure}

Figure \ref{fig:alpha} shows an ablation study done on $\alpha$ in Equation \ref{eqn:alpha}. We observed how the performance of \textbf{POP} and \textbf{NR-MOST} change as the value of $\alpha$ changes in the range of \{0.0001, 0.0002, ..., 0.0199, 0.0200\}. The plot on the left shows the results for \textbf{POP}. We can see that when $\alpha$ is too low, the influence of older popularity survives for too long that it degrades the performance. An easier way to understand the meaning of $\alpha$ is to look at its half life. Since the mass decays by $e^{-\alpha \Delta t}$, the time it takes for the mass to become half is $\Delta t = \frac{\log(2)}{\alpha}$. For example, when $\alpha = 0.0001$, the half-life is roughly 2 hours, which is too long to capture the recent trends accurately. Similarly, when $\alpha$ is too large (e.g. 0.02), its half life is too short (e.g. 34 seconds) to maintain the trend information. We found the sweet spot to be $\alpha = 0.0071$ (half life 97 seconds). For \textbf{NR-MOST} (plot on the right), we observed a similar pattern. However, the sweet spot was $\alpha=0.0015$ (half life 7 minutes). Also, the plot is noisier than the plot for \textbf{POP} since \textbf{NR-MOST} has other towers that interfere with the trend information. We included the performance of \textbf{NAML} for comparison. We can notice that the performance of \textbf{NAML} (and all other baselines) doesn't change with regard to $\alpha$ because it does not have a temporal factor in its model. \textbf{NR-MOST} underperforms \textbf{NAML} in two cases where $\alpha$ is extremely small (0.0001, 0.0002). But in all other cases it outperforms \textbf{NAML} by a large margin.

\subsubsection{Effect of number of blocks}
\label{section:numblocks}

\begin{figure}[H]
  \centering
  \includegraphics[width=\linewidth]{sections/figures/blocks.pdf}
  \caption{The effect of the number of blocks on the performance of \textbf{NR-MOST}.}
  \Description[Test Desc]{Test Description}
  \label{fig:blocks}
\end{figure}

To test the limit of performance gain with regard to the number of towers, we conducted the following ablation study. We defined \textbf{wpcstf} to be one \textbf{block}, then evaluated the performance of 1 to 5 \textbf{blocks} ($\textbf{(wpcstf)}^{\textbf{1}}$, ..., $\textbf{(wpcstf)}^{\textbf{5}}$). Figure \ref{fig:blocks} shows that after 2 \textbf{blocks}, the performance instead drops and saturates. We can conclude that too much towers sacrifice the performance since they become prone to overfitting.

==> sections/experiments_subsection/datasets.tex <==
% \begin{table}[t]
% \caption{Caption}
% \Description[Description]{Description}
% \label{tab:dataset}
% \begin{tabular}{@{}lrrrrr@{}}
% \toprule
% Dataset & Users   & News   & Clicks     & Avg. Length & Density \\ \midrule
% Small   & 11,812  & 53,111 & 665,550    & 56.35       & 0.106\% \\
% Mid     & 112,416 & 78,655 & 6,286,027  & 55.92       & 0.071\% \\
% Large   & 866,586 & 94,675 & 43,874,714 & 50.63       & 0.053\% \\ \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[t]
% \caption{Dataset Statistics}
% \Description[Description]{Description}
% \label{tab:dataset}
% \begin{tabular}{@{}l|rrr@{}}
% \toprule
%                                                             & \textbf{small}   & \textbf{mid}       & \textbf{large}      \\ \midrule
% \#users                                                     & 11,812  & 112,416   & 866,586    \\
% \#news                                                      & 53,111  & 78,655    & 94,675     \\
% \#clicks                                                    & 665,550 & 6,286,027 & 43,874,714 \\
% Avg. \#history                                              & 56.35   & 55.92     & 50.63      \\
% density                                                     & 0.106\% & 0.071\%   & 0.053\%    \\
% \begin{tabular}[c]{@{}l@{}}\#words per title\end{tabular}   & 9.19    & 9.15      & 9.12       \\
% \#categories                                                & 6       & 6         & 6          \\
% \#subcategories                                             & 55      & 57        & 57         \\ \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[t]
\caption{Dataset Statistics}
\Description[Description]{Description}
\label{tab:dataset}
\begin{tabular}{@{}l|rr@{}}
\toprule
                                                            & \textbf{Small}   & \textbf{Large}  \\ \midrule
\#users                                                     & 11,812  & 112,416   \\
\#news                                                      & 53,111  & 78,655    \\
\#clicks                                                    & 665,550 & 6,286,027 \\
Avg. \#history                                              & 56.35   & 55.92    \\
density                                                     & 0.106\% & 0.071\%  \\
\begin{tabular}[c]{@{}l@{}}\#words per title\end{tabular}   & 9.19    & 9.15     \\
\#categories                                                & 6       & 6        \\
\#subcategories                                             & 55      & 57        \\ \bottomrule
\end{tabular}
\end{table}

We conducted our experiments on real-world click logs from a large news service company. %\footnote{Unfortunately, we cannot publish the datasets for proprietary reasons}.
We randomly sampled the users and collected their history from December 6, 2020 to December 18, 2020 and their targets from December 19, 2020 to December 20, 2020. We created two datasets (i.e. \textbf{Small} and \textbf{Large}) by sampling 0.5\% and 5\% from the entire log respectively. The statistics for these datasets can be found in Table \ref{tab:dataset}.

We sorted the targets by their timestamps and split them by 8:1:1 to get train, validation, and test set respectively. For each clicked item, we have at most 45 negative items that weren't clicked by the user. %While in many settings these impression items are conveniently used as negative sets, we found that these negative sets do not reflect real-world environments faithfully and often lead to unfair model comparison. Since the impressions are already the result of the recommendation system in the service, they mostly contain items that more or less correspond to each user's preferences. For example, in one extreme case, we found that the impression items consisted of articles all with the same category that the user preferred. Training and evaluating the models with these negative sets can produce misleading results, and we have empirically proven this to be the case (we omit this analysis for the sake of space). Therefore, along with the 15 impression items, we added another 30 items to construct negative sets that better reflect the real-world environment. First, for each target, we sampled 15 items that were recently popular but weren't shown to or clicked by the user. Next, we sample another 15 items that have categories less preferred by the user. These 45 items are used as negative sets both for training and evaluation. At evaluation, we rank the positive and negative items by the model's output, then measure its quality by metrics such as NDCG@k, Recall@K, and AUC.
At evaluation, we rank the clicked item together with these negative items by the model's output, then measure its quality by metrics such as NDCG@k, Recall@k, and AUC.

==> sections/experiments_subsection/implementation_details.tex <==
In order to fairly evaluate the effectiveness of our method, we implemented \textbf{NR-MOST} \footnote{We will reveal our source code after the publication of this paper.} and all baselines in \texttt{PyTorch} \cite{pytorch} and experimented with the same device (Tesla M40). We used Bayesian optimization to find the optimal set of hyperparameters for each model using Weights \& Biases \cite{wandb}. As for common hyper-parameters, we searched for batch size within $\interval[{8,512]}$, length of user's history within \{10,20,...,90,100\}, length of words for each news article within \{10,20,30,40,50\}, learning rate within $\interval[{0.01,0.0001]}$ and dropout within $\interval[{0.1,0.9]}$. We searched for the number of attention heads within \{1,2,4,8,16\} for models that use attention operations. We searched within $\interval[{32,512]}$ for many hidden dimensions such as $d_{query}$ in additive attention, number of filters in CNN layers, and etc. We used the same set of pre-trained word embeddings with the embedding dimension of $d_{word} = 128$ for all models. These word embeddings were learned on the large corpus of news articles that were actually served by the company to provide better word representations and reduce OOV (out-of-vocabulary) rate.

For the sake of describing the combination of towers in \textbf{NR-MOST}, we introduce the following notations. First, we let \textbf{w}, \textbf{p}, \textbf{c}, \textbf{s}, \textbf{t}, and \textbf{f} each denote $\mathcal{T}^{word}$, $\mathcal{T}^{personal}$, $\mathcal{T}^{cat}$, $\mathcal{T}^{subcat}$, $\mathcal{T}^{trend}$ and $\mathcal{T}^{fresh}$ respectively. Then, we use a sequence of these letters to denote a specific combination. For example, \textbf{wpcstf} is equal to using one for each type of tower, and \textbf{wwppccssttff} is equal to using two for each. For brevity, we will sometimes write the latter as $\textbf{w}^\textbf{2}\textbf{p}^\textbf{2}\textbf{c}^\textbf{2}\textbf{s}^\textbf{2}\textbf{t}^\textbf{2}\textbf{f}^\textbf{2}$, or $\textbf{(wpcstf)}^\textbf{2}$.

We used the tower combination of $\textbf{w}^\textbf{2}\textbf{p}^\textbf{2}\textbf{c}^\textbf{2}\textbf{s}^\textbf{2}\textbf{t}^\textbf{2}\textbf{f}^\textbf{2}$ for performance comparison. We used $\alpha=0.001$, $\beta_1=0.01$, $\beta_2=0.001$, $\beta_3=0.0001$, $\beta_4=0.00001$, $d_{tr}=1024$, $d_{cat}=128$, $d_{subcat}=128$, and $d_{tvec}=128$. We searched for the optimal $d_{base}$, $d_{query}$ within $\interval[{256, 2 \times |v_*|}]$ and $\interval[{32, 512}]$ respectively.

==> sections/experiments_subsection/performance_comparison.tex <==
\input{sections/experiments_subsection/performance_table}

Table \ref{tab:performance} shows the performance of all models on our datasets. It also shows the relative improvement of the best performance (in \textbf{bold}) compared with the next best performance (in \underline{underline}). Among the baselines, \textbf{POP} performed the worst since it only considers the global popularity (trend) of the items and does not consider the personal preferences of the user. However, its performance is decent, showing that trend is a powerful signal by itself. Interestingly, \textbf{DSSM} performed better than \textbf{DeepFM} despite being a simple model that averages word embeddings. Since our word embeddings are pre-trained with the large corpus of news articles in the service, merely taking an average of those embeddings can still capture the semantics of the user's history and the candidate article to some extent. Surprisingly, \textbf{Weave\&Rec} underperforms \textbf{DSSM} and even \textbf{DeepFM}. Although other models such as \textbf{LSTUR}, \textbf{NAML} and \textbf{NPA} also use CNNs in their news encoders, the difference in \textbf{Weave\&Rec} is that it considers the sequence of word embeddings as a 2D matrix and as a result divide each word embedding into small windows. This could lead to inept representations of news articles. Moreover, it has the same problem for user representations since it applies a rigid 3D CNNs on the users' history.

Models with more advanced news encoders and user encoders outperform the models mentioned above. First, \textbf{NPA} outperforms those models by using a personalized attention module in both its news encoder and user encoder. However, since users' interactions are very sparse in the news domain, using an ID-based embedding to directly model the users' interests can lead to overfitting. \textbf{NRMS} performs better than \textbf{NPA} by using an additional self-attention layer in both its news encoder and user encoder. However, since its news encoder only utilizes the textual features of news articles, it fails to capture their categorical aspects. Therefore, both \textbf{LSTUR} and \textbf{NAML} outperform \textbf{NRMS} by including the categorical features in their news encoders. \textbf{NAML} outperforms \textbf{LSTUR} which shows that user encoders using attention operations perform better than those that use RNNs.

Finally, it is clear that our proposed framework outperforms all of the baselines. More specifically, in terms of Recall@5 and NDCG@5, its performance improves by 20.17\% and 20.17\% in \textbf{Small} dataset and by 22.75\% and 26.14\% in \textbf{Large} dataset compared against the strongest baseline model. We attribute the excellence of \textbf{NR-MOST} to its (a) novel use of semantic, categorical, and temporal features, and (b) the combination and interaction of multiple specialized towers. In the next section we study in detail the effect of each of these components.

==> sections/experiments_subsection/performance_table.tex <==
% dataset description & statistics

% performance table
% https://www.tablesgenerator.com
\begin{table*}[]
\caption{Performance Comparison.}
\Description[Description]{Description}
\label{tab:performance}

% last updated: 5/12 02:15
\begin{tabular}{@{}llcccccccccr@{}}
\toprule
Dataset                & Metric     & POP    & Weave\&Rec    & DeepFM   & DSSM      & NPA    & NRMS   & LSTUR  & NAML               & NR-MOST          & Improv.    \\ \midrule
\multirow{5}{*}{Small} & Recall@5   & 0.1771 & 0.2732        & 0.3029   & 0.3389    & 0.3454 & 0.3589 & 0.3886 & \underline{0.4174} & \textbf{0.5016}  & 20.17\%    \\
                       & Recall@10  & 0.3165 & 0.4599        & 0.4768   & 0.5449    & 0.5545 & 0.5777 & 0.6050 & \underline{0.6314} & \textbf{0.7276}  & 15.24\%    \\
                       & NDCG@5     & 0.1174 & 0.1684        & 0.1907   & 0.2116    & 0.2189 & 0.2356 & 0.2471 & \underline{0.2796} & \textbf{0.3360}  & 20.17\%    \\
                       & NDCG@10    & 0.1618 & 0.2284        & 0.2463   & 0.2786    & 0.2869 & 0.3063 & 0.3165 & \underline{0.3482} & \textbf{0.4089}  & 17.43\%    \\
                       & AUC        & 0.6309 & 0.7149        & 0.7332   & 0.7571    & 0.7559 & 0.7757 & 0.7993 & \underline{0.8164} & \textbf{0.8493}  & 4.03\%     \\ \midrule
\multirow{5}{*}{Large} & Recall@5   & 0.2080 & 0.2950        & 0.2849   & 0.3228    & 0.3492 & 0.3842 & 0.3940 & \underline{0.4273} & \textbf{0.5245}  & 22.75\%    \\
                       & Recall@10  & 0.3223 & 0.4884        & 0.5036   & 0.5520    & 0.5589 & 0.5932 & 0.6111 & \underline{0.6325} & \textbf{0.7284}  & 15.16\%    \\
                       & NDCG@5     & 0.1381 & 0.1839        & 0.1799   & 0.2005    & 0.2317 & 0.2576 & 0.2584 & \underline{0.2858} & \textbf{0.3605}  & 26.14\%    \\
                       & NDCG@10    & 0.1747 & 0.2458        & 0.2497   & 0.2740    & 0.2990 & 0.3247 & 0.3281 & \underline{0.3518} & \textbf{0.4262}  & 21.15\%    \\
                       & AUC        & 0.6404 & 0.7383        & 0.7633   & 0.7653    & 0.7790 & 0.7908 & 0.8092 & \underline{0.8197} & \textbf{0.8550}  & 4.31\%     \\ 
% Dataset                & Metric     & POP    & DeepFM   & DSSM      & Weave\&Rec    & LSTUR  & NPA    & NRMS   & NAML               & NR-MOST          & Improv.    \\ \midrule
% \multirow{5}{*}{Small} & Recall@5   & 0.1771 & 0.3029   & 0.3389    & 0.2732        & 0.3886 & 0.3454 & 0.3589 & \underline{0.4174} & \textbf{0.5016}  & 20.17\%    \\
%                       & Recall@10  & 0.3165 & 0.4768   & 0.5449    & 0.4599        & 0.6050 & 0.5545 & 0.5777 & \underline{0.6314} & \textbf{0.7276}  & 15.24\%    \\
%                       & NDCG@5     & 0.1174 & 0.1907   & 0.2116    & 0.1684        & 0.2471 & 0.2189 & 0.2356 & \underline{0.2796} & \textbf{0.3360}  & 20.17\%    \\
%                       & NDCG@10    & 0.1618 & 0.2463   & 0.2786    & 0.2284        & 0.3165 & 0.2869 & 0.3063 & \underline{0.3482} & \textbf{0.4089}  & 17.43\%    \\
%                       & AUC        & 0.6309 & 0.7332   & 0.7571    & 0.7149        & 0.7993 & 0.7559 & 0.7757 & \underline{0.8164} & \textbf{0.8493}  & 4.03\%     \\ \midrule
% \multirow{5}{*}{Large} & Recall@5   & 0.2080 & 0.2849   & 0.3228    & 0.2950        & 0.3940 & 0.3492 & 0.3842 & \underline{0.4273} & \textbf{0.5245}  & 22.75\%    \\
%                       & Recall@10  & 0.3223 & 0.5036   & 0.5520    & 0.4884        & 0.6111 & 0.5589 & 0.5932 & \underline{0.6325} & \textbf{0.7284}  & 15.16\%    \\
%                       & NDCG@5     & 0.1381 & 0.1799   & 0.2005    & 0.1839        & 0.2584 & 0.2317 & 0.2576 & \underline{0.2858} & \textbf{0.3605}  & 26.14\%    \\
%                       & NDCG@10    & 0.1747 & 0.2497   & 0.2740    & 0.2458        & 0.3281 & 0.2990 & 0.3247 & \underline{0.3518} & \textbf{0.4262}  & 21.15\%    \\
%                       & AUC        & 0.6404 & 0.7633   & 0.7653    & 0.7383        & 0.8092 & 0.7790 & 0.7908 & \underline{0.8197} & \textbf{0.8550}  & 4.31\%     \\ 
\bottomrule
\end{tabular}
\end{table*}

==> sections/formulation.tex <==
The problem of news recommendation can be formulated as follows. Let $\mathcal{U}$ be a set of users, $\mathcal{N}$ be a set of news articles, $\mathcal{C}$ be a set of categories, $\mathcal{S}$ be a set of subcategories, and $\mathcal{V}$ be a set of vocabularies. The history of each user $u \in \mathcal{U}$ can be represented as $\mathcal{N}^u=[(n^u_1, t^u_1), ..., (n^u_{|\mathcal{N}^u|}, t^u_{|\mathcal{N}^u|})]$ where $n^u_k \in \mathcal{N}$ is a $k$th news article clicked by $u$ at timestamp $t^u_k$. Similarly, all users who clicked on an article $n$ can be collected as $\mathcal{U}^n=[(u^n_1, t^n_1), ..., (u^n_{|\mathcal{U}^n|}, t^n_{|\mathcal{U}^n|})]$. We assume that the timestamps are sorted in an increasing order in both cases.

Each news article $n \in \mathcal{N}$ is associated with multiple features. First, it has textual features such as a title and a body, which can each be tokenized into a sequence of words (e.g. $\texttt{title}_n = [w_1, ..., w_{|\texttt{title}_n|}]$). We assume that all words are included in our vocabulary $\mathcal{V}$, and that we have pre-trained embeddings for the words in our vocabulary ($E^V \in \mathbb{R}^{|V| \times d_{word}}$ where $d_{word}$ is the word embedding dimension). A news article also owns a categorical feature such as a category $\texttt{cat}_n \in \mathcal{C}$ (e.g. sports), and a subcategory $\texttt{subcat}_n \in \mathcal{S}$ (e.g. basketball). Finally, it also has temporal features such as \texttt{trend} and \texttt{freshness}. The definition of these temporal features will be explained in detail in section \ref{trendsection}.

Given the above, our goal is to recommend a set of news articles for a user at target timestamp. More specifically, at target time $t_{target}$, given $K$ candidate news articles $[cand_1, ..., cand_{K}]$ and the user's history $[n^u_1, ..., n^u_{|N^u|}]$, our goal is to rank those candidates in the order of the user's estimated preferences. 

==> sections/method.tex <==
\subsection{NR-MOST Framework}
\input{sections/method_subsections/framework}

\subsection{Semantic Towers}
\input{sections/method_subsections/semantic}

\subsection{Categorical Towers}
\input{sections/method_subsections/categorical}

\subsection{Temporal Towers}
\input{sections/method_subsections/temporal}

\subsection{Discussion}
\input{sections/method_subsections/discussion}

==> sections/method_subsections/categorical.tex <==
In this subsection we introduce two types of categorical towers: $\mathcal{T}^{cat}$ and $\mathcal{T}^{subcat}$. Their designs are quite straightforward in that they are identical to $\mathcal{T}^{word}$. However, we replace the news encoder with the following. Recall that each news article $n$ is endowed with categorical features such as a category $\texttt{cat}_n \in \mathcal{C}$ (e.g. sports), or a subcategory $\texttt{subcat}_n \in \mathcal{S}$ (e.g. basketball). In $\mathcal{T}^{cat}$, for example, an embedding table $E^{\mathcal{C}} \in \mathbb{R}^{|\mathcal{C}| \times d_{\texttt{cat}}}$ is employed where each entry is a learnable vector for each category and $d_{\texttt{cat}}$ is its dimension. Using $E^{\mathcal{C}}$, a representation for each news $n$ is computed as a simple embedding look-up operation for its category $\texttt{cat}_n$. The rest of the tower (e.g. user encoder) remains the same. In this view, the user representation can be said to summarize the user's preferences for categories, which can be compared with the category vectors of candidate articles for similarity. $\mathcal{T}^{subcat}$ can be designed identically for subcategories.

==> sections/method_subsections/discussion.tex <==
Although we settle for these few number of designs for each type of feature, our framework is extensible to novel designs and types of features. Ablation shows that doing so will continue to improve the performance. However, note that we stress the novelty of our overall framework more than the novelty of each tower.


==> sections/method_subsections/framework.tex <==
% \begin{figure*}[!htbp]
%   \centering
%   \includegraphics[width=0.9\linewidth]{sections/figures/fig2_our_framework.pdf}
%   \caption{(a)(b)(c)(d)(e)}
%   \Description[Test Desc]{Test Description}
%   \label{fig:ourframework}
% \end{figure*}

Our framework is illustrated in Figure \ref{fig:ourframework}. The figure describes how the click probability $\hat{y}_k$ for the candidate news $cand_k$ is generated. For brevity, we only included a single candidate item in the figure, but in reality the same operation is applied to all $K$ candidates. In short, our framework consists of multiple "towers" where each tower serves a special purpose.

We suppose that there are in total $T = T_{sem} + T_{cat} + T_{temp}$ number of towers that each work on semantic (\textbf{red}, Figure \ref{fig:ourframework} (a)), categorical (\textbf{blue}, Figure \ref{fig:ourframework} (b)) or temporal (\textbf{green}, Figure \ref{fig:ourframework} (c)) features respectively. For simplicity, let us denote each tower as $\mathcal{T}_i$ ($i \in [1, T]$). A tower $\mathcal{T}$ does the following operation:

\begin{equation}
    \mathcal{T}(user, news, t_{target}) = (s,v)
\end{equation}
which takes a user, a news article, and a target timestamp to output a scalar value $s$ and a vector $v$. Here, $s$ serves as the score and $v$ serves as output features generated by the tower.

We first concatenate all vector outputs

\begin{equation}
    v_* = v_1 \oplus ... \oplus v_T
\end{equation}

then feed it to the interaction MLP layer (Figure \ref{fig:ourframework} (d)) to learn their interactions as follows.

\begin{align}
    v_*^{1} &= \textrm{ReLU}(W^{1}_{int} v_* + b^{1}_{int}) \\
    v_*^{2} &= \textrm{ReLU}(W^{2}_{int} v_*^1 + b^{2}_{int}) \\
    v_*^{3} &= \textrm{ReLU}(W^{3}_{int} v_*^2 + b^{3}_{int}) \\
    s_{int} &= W^{4}_{int} v_*^3 + b^{4}_{int}
\end{align}

where $W^{1}_{int} \in \mathbb{R}^{d_{base} \times |v_*|}$, $b^{1}_{int} \in \mathbb{R}^{d_{base}}$, $W^{2}_{int} \in \mathbb{R}^{\frac{d_{base}}{2} \times d_{base}}$, $b^{2}_{int} \in \mathbb{R}^{\frac{d_{base}}{2}}$, $W^{3}_{int} \in \mathbb{R}^{\frac{d_{base}}{4} \times \frac{d_{base}}{2}}$, $b^{3}_{int} \in \mathbb{R}^{\frac{d_{base}}{4}}$, $W^{4}_{int} \in \mathbb{R}^{1 \times \frac{d_{base}}{4}}$, $b^{4}_{int} \in \mathbb{R}^{1}$ are learnable parameters and $d_{base}$ controls the width of the MLP.

Next, we concatenate the result $s_{int}$ with the scalar outputs from all towers

\begin{equation}
    s_* = s_1 \oplus ... \oplus s_T \oplus s_{int}
\end{equation}

then do a weighted sum (Figure \ref{fig:ourframework} (e)) to get the click probability

\begin{equation}
    \hat{y}_k = W_{score} \times s_* + b_{score}
\end{equation}

where $W_{score} \in \mathbb{R}^{1 \times (T+1)}$, $b_{score} \in \mathbb{R}^{1}$ are learnable parameters.

Note that in this perspective, a typical framework (Figure \ref{fig:typical}) would be equivalent to using only one tower (e.g. $T_1$), and directly using its scalar output (e.g. $s_1$) as the click probability. In contrast, in \textbf{NR-MOST}, more than one specialized towers contribute to the final prediction, resulting in boosted model capacity by resolving the information bottleneck that existed in previous frameworks. Moreover, interaction MLP layer (Figure \ref{fig:ourframework} (d)) further enhances the model's performance since it can learn complicated interactions between multiple features of the candidate news and the user (e.g. how likely is the user $u$ to conform to the currently trendy item $n$ given $u$ and $n$'s semantic/categorical information?)

In the following subsections, we will describe in detail the inner workings of each specialized tower.

==> sections/method_subsections/semantic.tex <==
Semantic towers deal with the textual semantics of news articles and the user's semantic interests. In this section we introduce two types of semantic towers: $\mathcal{T}^{word}$ and $\mathcal{T}^{personal}$.

The structure of $\mathcal{T}^{word}$ is illustrated in Figure \ref{fig:towers} (a). It adopts the same news encoder and user encoder devised in NRMS~\cite{NRMS}. In NRMS, both the news encoder and the user encoder use the same type of operations. More specifically, they use two kinds of attention operations: multi-headed self-attention~\cite{TRANSFORMER} and additive attention \cite{additive}. The former is defined in \cite{TRANSFORMER, NRMS} (we omit the definition for the sake of space), and the latter is defined as follows:

\begin{align}
    &\textrm{Additive}(x) = \sum_{i}{\alpha_i \times x_i} \\
    &\alpha = \textrm{softmax}(a) \\
    &a_i = q_{add}^T \textrm{tanh}(W_{add}x_i + b_{add}) \label{eqn:additiveattnweights}
\end{align}

where $q_{add} \in \mathbb{R}^{d_{query}}, W_{add} \in \mathbb{R}^{d_{query} \times d}, b_{add} \in \mathbb{R}^{d_{query}}$ are learnable parameters and $d_{query}$ is the dimension of the query vector $q_{add}$. With these operations, one can build an encoder that takes an input of shape $\mathbb{R}^{N \times d}$ and outputs a vector of shape $\mathbb{R}^{d}$:

\begin{equation}
    \textrm{Enc}_{\textrm{(Mult, Add)}}(x) = \textrm{Additive}(\textrm{Multihead}(x))
\end{equation}

This encoder is used both as news encoder and user encoder as shown in Figure \ref{fig:towers} (a). First, a representation $r$ of a news article $n$ is computed as 

\begin{equation}
    r = \textrm{Enc}_{\textrm{(Mult, Add)}}([e_1, ..., e_{|\texttt{title}_n|}])
\end{equation}
where $e_k$ is a word embedding from $E^V$ for the word $w_k$ in the title of $n$. With this method we get the representation $r_{cand_k}$ for the candidate $cand_k$, and the representations $[r^u_1, ..., r^u_{|N^u|}]$ for the user's history $[n^u_1, ..., n^u_{|N^u|}]$. Next, we use the same operation (with different parameters) to get the user's representation as

\begin{equation}
    r_u = \textrm{Enc}_{\textrm{(Mult, Add)}}([r^u_1, ..., r^u_{|N^u|}]) \label{eqn:ru}
\end{equation}

Finally, the scalar and vector output of this tower are each obtained by the dot product and the concatenation of $r_{cand_k}$ and $r_u$:

\begin{equation}
    \mathcal{T}^{word}(user, news, t_{target}) = (r_{cand_k} \odot r_u, r_{cand_k} \oplus r_u)
\end{equation}

Note that in our case, an additional vector output is produced, whereas in NRMS~\cite{NRMS}, only the scalar output is produced. Here, the scalar output measures the similarity between the semantic representations of the candidate news and the user, while the vector output preserves those two representations. The former contributes directly to the click prediction while the latter is used as input in the interaction MLP layer.

In addition, we devised another semantic tower called $\mathcal{T}^{personal}$. Since user’s news reading behavior can be affected by the trend, it is important to incorporate the trendiness of clicked items in order to extract true semantic interests of the user. $\mathcal{T}^{personal}$ uses the same news encoder as in $\mathcal{T}^{word}$. However, we replace its user encoder with $\textrm{Enc}_{\textrm{(Mult, TrAdd)}}$ where $\textrm{TrAdd}$ ($\textrm{Trend}$ $\textrm{Additive}$) is another operation we devised to incorporate the trend information. Recall that $\textrm{Additive}$ is used to combine the representations of the user's history $[r^u_1, ..., r^u_{|N^u|}]$ into a single vector $r_u$ by additive attention operation (Equation \ref{eqn:ru}). However, in $\textrm{TrendAdditive}$, we replace Equation (\ref{eqn:additiveattnweights}) with the following:

\begin{align}
    a^0_i &= \log(1 + \texttt{trend}(n^u_i, t^u_i)) \label{eq:trmlpbegin} \\
    a^1_i &= ReLU(W^1_{tr} a^0_i + b^1_{tr}) \\
    a^2_i &= ReLU(W^2_{tr} a^1_i + b^2_{tr}) \\
    a^3_i &= ReLU(W^3_{tr} a^2_i + b^3_{tr}) \\
    a_i &= (W^4_{tr} a^3_i + b^4_{tr}) \label{eq:trmlpend}
\end{align}



where $W^{1}_{tr} \in \mathbb{R}^{d_{tr} \times 1}$, $b^{1}_{tr} \in \mathbb{R}^{d_{tr}}$, $W^{2}_{tr} \in \mathbb{R}^{d_{tr} \times d_{tr}}$, $b^{2}_{tr} \in \mathbb{R}^{d_{tr}}$, $W^{3}_{tr} \in \mathbb{R}^{d_{tr} \times d_{tr}}$, $b^{3}_{tr} \in \mathbb{R}^{d_{tr}}$, $W^{4}_{tr} \in \mathbb{R}^{1 \times d_{tr}}$, $b^{4}_{tr} \in \mathbb{R}^{1}$ are learnable parameters, $d_{tr}$ is the width of the MLP, and \texttt{trend} is a temporal feature that will be defined in section \ref{trendsection}. For now, it is enough to note that the attention score for each historical item $n^u_i$ is determined not by its semantic representation $r^u_i$ but by its \texttt{trend} score at the time of its click $t^u_i$. This allows the neural network to learn a trend-aware view on the user's historical behaviors. For example, if the network learns to give more weights to the items that were less trendy at the time of user's click, then it might learn more personal preferences of the user.

==> sections/method_subsections/temporal.tex <==
\label{trendsection}

Popularity is a very important signal in almost all recommendation problem settings. This is even more so in the news domain where the value of an article is determined to a large extent by its current popularity (trend), and its timeliness (freshness). To be able to efficiently acquire these attributes for any article at any point in time, we came up with the following method. First, for any article $n$, we collect all users who clicked on $n$ and their click timestamps: $U^n = [(u^n_1, t^n_1), ..., (u^n_{|U^n|}, t^n_{|U^n|})]$. Next, we define the mass $m$ of $k$th click $(u^n_k, t^n_k)$ at time $t$ to be the following:

\begin{equation}
    m(n, t, k) =
\begin{cases}
    e^{-\alpha (t - t^n_k)},& \textrm{if } t \geq\ t^n_k \label{eqn:alpha} \\ 
    0,              & \textrm{otherwise}
\end{cases}
\end{equation}

In other words, every click generates a mass of $1$ at the time of click, which gets exponentially decayed as time passes. $\alpha$ is a parameter that can be adjusted to control the lifespan of the masses. With this, one can define the trend score (\texttt{trend}) of $n$ at $t$ as:

\begin{equation}
    \texttt{trend}(n, t) = \sum_{k}{m(n, t, k)}
\end{equation}

Note that this definition is computationally efficient both at offline/online settings because masses can be cumulatively maintained as a single value at any timestamp with easy updates. Yet it is also very effective because it summarizes how trendy $n$ is at any point in time $t$ as a scalar value. With this useful information, one can easily devise a tower $\mathcal{T}^{trend}$ shown in Figure \ref{fig:towers} (b).

In $\mathcal{T}^{trend}$, only the trend score $trend(cand_k, t_{target})$ is used as input. It is processed in the same fashion as Equations \ref{eq:trmlpbegin}-\ref{eq:trmlpend}. It is first scaled down by $log(1+x)$ operation since the value of the trend score can be very high which is unsuitable for neural networks. Then it is processed by MLP layers to learn a non-linear function. However, in this case, the output dimension of Equation \ref{eq:trmlpend} is extended from 1 to 1+$d_{tvec}$ so that the first value can be used as the scalar output and the rest as the vector output of length $d_{tvec}$.

Similarly, one can define the freshness score (\texttt{fresh}) of $n$ at $t$ as:

\begin{equation}
    \texttt{fresh}(n, t) = [e^{-\beta_1 (t - t^n_1)}, ..., e^{-\beta_f (t - t^n_1)}]
\end{equation}

In other words, an article's freshness at time $t$ is defined as its temporal distance from the first click that ever occurred, exponentially decayed by different factors $\beta_1, ..., \beta_f$. Similar to $\mathcal{T}^{trend}$, by feeding these values into MLP layers (without $log(1+x)$ operation in the beginning), one gets another tower $\mathcal{T}^{fresh}$.

The scalar outputs from these temporal towers deliver important signals for candidate articles such as trendiness and freshness, which greatly improves the recommendation performance. The vector outputs which also hold these signals in vector forms further improve the performance by being mixed with vector outputs from other types of towers in the interaction MLP layer.

==> sections/relworks_subsections/disentangled.tex <==
% Disentangling approaches

% Side information를 사용하는 연구

%% Fashion rec 쪽은 category 보다는 visual info를 많이 사용 (multi-modal)
%%% https://scholar.google.co.kr/scholar?as_ylo=2017&q=fashion+recommendation+multimodal&hl=ko&as_sdt=0,5

%% Movie rec 에서 genre를 사용하는 연구들이 있음
%%% https://scholar.google.co.kr/scholar?as_ylo=2017&q=movie+recommendation+genre&hl=ko&as_sdt=0,5

%% POI rec 에서 category를 사용하는 연구들이 있음
%%% https://scholar.google.co.kr/scholar?as_ylo=2020&q=poi+recommendation+category&hl=ko&as_sdt=0,5

==> sections/relworks_subsections/seq.tex <==
!!!!!!!!!COPIED FROM MEANTIME. NEEDS FIX!!!!!!!!!!!!!!!!
Sequential recommendation aims to suggest relevant items based on the user's sequential history. Markov-chain based methods~\cite{SIMILARITYMC, MCAULEYMC2016, TRANSREC, he2016fusing} assume that users' behaviors are affected only by their last few behaviors. FPMC~\cite{rendle2010factorizing} merges Markov-chains with matrix factorization method for next-basket recommendation. Since the first suggestion by GRU4Rec~\cite{GRU4Rec}, many RNN-based methods~\cite{hidasi2018recurrent, RNN4Rec, HIERARCHICALGRU4REC, DREAM, wu2017recurrent, wu2017sequential, DINEVOLUTION} brought the success of RNN into item sequence understanding. To overcome the strong order constraint of RNN models, CNN-based methods~\cite{CASER, CNNGENERATIVE, HIERARCHICALCNN} were proposed. Some works adopted graph neural network (GNN) to understand user's session as a graph~\cite{SESSIONGNN}.

As for attention mechanisms, NARM~\cite{NARM} and STAMP~\cite{STAMP} incorporated vanilla attention mechanism with RNN. More recently, SASRec~\cite{SASRec} successfully employed self-attention mechanism, which was a huge success in NLP areas~\cite{TRANSFORMER, BERT, TRANSFORMER-XL, XLNET}. BERT4Rec~\cite{BERT4Rec} improved SASRec by adopting Transformer~\cite{TRANSFORMER} and Cloze-task based training method. TiSASRec~\cite{TISASRec} enhanced SASRec by merging timestamp information into self-attention operations. Our work seeks to further expand this trend by suggesting a novel model architecture that uses multiple types of temporal embeddings  and self-attention operations to better capture the diverse patterns in user's behaviors.

==> sections/relworks_subsections/temporal.tex <==
!!!!!!!!!COPIED FROM MEANTIME. NEEDS FIX!!!!!!!!!!!!!!!!

Since temporal information hold contextual information, they can be very crucial for recommendation performance. TimeSVD++ and BPTF~\cite{TIMESVD++, BPTF} adopted time factor into the matrix factorization method, and TimeSVD++ was one of the main contributions for the winning of Netflix Grand Prize~\cite{NETFLIXPRIZE}.
%Bayesian Probabilistic Tensor Factorization (BPTF)~\cite{BPTF} added time constraints when factorizing the tensors. However, these works were limited to the traditional factorization setting where the sequential nature of data is ignored. Meanwhile,
Time-LSTM~\cite{TIMELSTM} equipped LSTMs with several forms of time gates to better model the time intervals in user's interaction sequence. Recently, CTA~\cite{CTA} used multiple parametrized kernel functions on temporal information to calibrate the self-attention mechanism.

Add MEANTIME \cite{MEANTIME}.

==> sections/relworks_subsections/user.tex <==
Deep learning methods were shown to be much more effective than traditional methods in terms of user modeling. For example, Okura et al. \cite{Okura} reported significant performance improvement over traditional temporal methods such as time-decay when they used Recurrent Neural Networks (RNNs) to model user behaviors. In fact, since GRU4Rec~\cite{GRU4Rec} was first proposed, many sequential recommendation methods employed RNN to benefit from its sequence understanding capability~\cite{hidasi2018recurrent, RNN4Rec, HIERARCHICALGRU4REC, DREAM, wu2017recurrent, wu2017sequential, DINEVOLUTION}. The same trend occurred in the news domain for user modeling~\cite{song2016, Okura, kumar2017, HRAM, an2019, zhu2019, zhang2019a, park2017deep}.
Some found Convolutional Neural Networks (CNNs) to be useful~\cite{Weave, FIM}. For example, Weave\&Rec~\cite{Weave} applied 3D CNN to the user's behavior sequence where each item was represented as a 2D matrix comprised of word embeddings.
More recently, prevalent usage of attention mechanisms were witnessed in recommendation models. In sequential recommendation, following the huge success of transformers in NLP~\cite{TRANSFORMER, BERT, TRANSFORMER-XL, XLNET}, models such as SASRec~\cite{SASRec}, BERT4Rec~\cite{BERT4Rec} and etc.~\cite{TISASRec, MEANTIME} fully adopted attention techniques, in contrast to previous models where attention was merely a part of the model~\cite{NARM, STAMP}. The same was true for user modeling in news domain~\cite{NRMS, NAML, NPA, DKNwang2018a, zhu2019, zhang2019a, wu2021feedrec, MMRec, wu2021empowering}. For example, models such as NRMS~\cite{NRMS}, NAML~\cite{NAML} and NPA~\cite{NPA} all used similar attention operations to combine the user's history into a single representation. However, we observed that there are two major limitations in most of the previous approaches. First, they usually combine the user's history into a single representation which can be a bottleneck when trying to capture the user's diverse interests. Second, their representations usually remain static regardless of the time of recommendation, which can hinder the model's performance in a highly dynamic environment such as news service. Our work seeks to improve user modeling methods in these aspects.
